Koopman and Perron-Frobenius Operators on reproducing kernel Banach spaces

Koopman and Perron-Frobenius operators for dynamical systems have been getting popular in a number of fields in science these days. Properties of the Koopman operator essentially depend on the choice of function spaces where it acts. Particularly the case of reproducing kernel Hilbert spaces (RKHSs) draws more and more attention in data science. In this paper, we give a general framework for Koopman and Perron-Frobenius operators on reproducing kernel Banach spaces (RKBSs). More precisely, we extend basic known properties of these operators from RKHSs to RKBSs and state new results, including symmetry and sparsity concepts, on these operators on RKBS for discrete and continuous time systems.

==> refs_journal.tex <==
@Misc{RKHSGlobalOptimization,
  author = {Rudi, A. and Marteau-Ferey, U. and Bach, F.},
  title = {Finding Global Minima via Kernel Approximations},
  year  = 2020,
  eprintclass = {math.NA},
  eprint  =	 {2012.11978}
}

@Article{AA17,
  author = {Abanin, A. V. and Abanina, T. I.},
  title = {Composition operators on Hilbert spaces of entire function},
  journal =	{Russ Math.},
  volume  =	61,
  year    = 2017,
  pages   =	{1--4}
}

@Book{RKHSProbability,
  author = {Berlinet, A. and Thomas-Agnan, C.},
  title = {Reproducing kernel Hilbert spaces in probability and statistics},
  publisher = {Springer Science \& Business Media},
  year    = 2011
}

@Book{Brezis,
  author = {Brezis, H.},
  title = {Functional Analysis, Sobolev Spaces and Partial DifferentialzEquations},
  publisher = {Springer-Verlag New York},
  year    = 2011
}

@Article{CCG,
  author = {Chacon, G. A. and Chacon, G. R. and Gimenez, J.},
  title = {Composition operators on spaces of entire functions},
  journal =	{Proc. Amer. Math. Soc.},
  volume  =	135,
  year    = 2007,
  pages   =	{2205--2218}
}

@Article{CMS,
  author = {Carswell, B. and MacCluer, B. D. and Schuster, A.},
  title = {Composition operators on the Fock space},
  journal =	{Acta Sci. Math.},
  volume  =	69,
  year    = 2003,
  pages   =	{871--887}
}

@Book{CompOpAnalyticFunctions,
  author = {Cowen, C. and Maccluer, B.},
  title = {Composition Operators on Spaces of Analytic Functions},
  publisher = {CRC press},
  year    =1995
}

@Article{DasSpectrum,
  author = {Das, S. and Giannakis, D.},
  title = {Koopman spectra in Reproducing kernel Hilbert spaces},
  journal =	{Applied and Computational Harmonic Analysis},
  volume  =	49,
  number  =	2,
  year    = 2018,
  pages   =	{573--607}
}

@article{mezic2020spectrum,
  title={Spectrum of the Koopman operator, spectral expansions in functional spaces, and state-space geometry},
  author={Mezi{\'c}, Igor},
  journal={Journal of Nonlinear Science},
  volume={30},
  number={5},
  pages={2091--2145},
  year={2020},
  publisher={Springer}
}


@Article{DKL17,
  author = {Doan, M.-L. and Khoi, L.-H. and Le, T.},
  title = {Composition operators on Hilbert spaces of entire functions of several variables},
  journal =	{Integral Equ. Oper. Theory},
  volume  =	88,
  number  =	3,
  year    = 2017,
  pages   =	{301--330}
}

@Book{EngelNagel,
  author = {Engel, K.-J. and Nagel, R.},
  title = {A Short Course on Operator Semigroups},
  publisher = {Berlin Heidelberg: Springer Science \& Business Media},
  year    = 2006
}

@Article{Das,
  author = {Das, S. and Giannakis, D.},
  title = {Delay-Coordinate Maps and the Spectra of Koopman Operators},
  journal =	{Journal of Statistical Physics},
  volume  =	175,
  number  =	4,
  year    = 2019,
  pages = {1107–-1145}
}

@Article{HIIK,
  author = {Hashimoto, Y. and Ishikawa, I. and Ikeda, M. and Kawahara, Y.},
  title = {Krylov Subspace Method for Nonlinear Dynamical Systems with random noises},
  journal =	{J. Mach. Learn. Res.},
  volume  =	21,
  year    = 2020,
  pages   =	{1--29}
}
\bibitem{HIIK}
Y.\ Hashimoto,  I.\ Ishikawa, M.\ Ikeda, Y.\ Kawahara,
Krylov Subspace Method for Nonlinear Dynamical Systems with random noises,
{\it J. Mach. Learn. Res.}, {\bf 21}, 2020, 1--29.

  
@article{MilanRoA,
  title={Convex Computation of the Region of Attraction of Polynomial Control Systems},
  author={Henrion, Didier and Korda, Milan},
  journal={IEEE Transactions on Automatic Control},
  volume={59},
  number={2},
  pages={297--312},
  year={2014},
  publisher={TAC}
}

@article{KernelsInMachineLearning,
  author = {Hofmann, T. and Scholkopf, B. and Smola, A.J.},
  title = {Kernel methods in machine learning},
  journal =	{The Annals of Statistics},
  volume  =	36,
  number  =	3,
  year    = 2008,
  pages   =	{1171--1220}
}

@article{IIS20,
  author = {Ikeda, M. and Ishikawa, I. and Sawano, Y.},
  title = {Composition operators on reproducing kernel Hilbert spaces with analytic positive definite functions},
  journal =	{Journal of Mathematical Analysis and Applications},
  volume  =	{511},
  number  =	{1},
  year    = {2022},
  pages   =	{126048}
}

@Misc{IsaoBoundedCompOp,
  author = {Ishikawa, I.},
  title = {Bounded weighted composition operators on functional quasi-Banach spaces and stability of dynamical systems},
  year = 2021,
  eprintclass = {math.NA},
  eprint  =	 {2105.04280}
}

@Article{IFIHK,
  author = {Ishikawa, I. and Fujii, K. and Ikeda, M. and Hashimoto, Y. and Kawahara, Y.},
  title = {Metric on Nonlinear Dynamical Systems with Perron--Frobenius Operators},
  journal =	{Adv. Neural Inf. Process. Syst.},
  volume  =	31,
  year    = 2018,
  pages   =	{911–-919}
}

@Article{Kawahara16,
  author = {Kawahara, Y.},
  title = {Dynamic Mode Decomposition with Reproducing Kernels for Koopman Spectral Analysis},
  journal =	{Adv. Neural Inf. Process.~Syst.},
  volume  =	29,
  year    = 2016,
}

@Book{Katznelson-text-04,
  author = {Katznelson, Y.},
  title = {An Introduction to Harmonic Analysis},
  publisher = {Cambridge University Press},
  year    = 2004
}

@Article{KernelMeanEmbedding,
  author = {Klus, S. and Schuster, I. and Muandet, K.},
  title = {Eigendecompositions of Transfer Operators in Reproducing Kernel Hilbert Spaces},
  journal =	{Journal of Nonlinear Science},
  volume  =	30,
  year    = 2020,
  pages   =	{283–-315}
}

@article{Milan14,
  title={Convex computation of the maximum controlled invariant set for polynomial control systems},
  author={Korda, Milan and Henrion, Didier and Jones, Colin N},
  journal={SIAM Journal on Control and Optimization},
  volume={52},
  number={5},
  pages={2944--2969},
  year={2014},
  publisher={SIAM}
}

@Article{KoopmanControlMilan,
  author = {Korda, M. and Mezi\'{c}, I.},
  title = {Linear predictors for nonlinear dynamical systems: Koopman operator meets model predictive control},
  journal =	{Automatica},
  volume  =	93,
  year    = 2018,
  pages   =	{149--160}
}

@Misc{RKBSUnified,
  author = {Lin, R. and Zhang, H. and Zhang, J.},
  title = {On reproducing kernel Banach spaces: Generic definitions and unified framework of constructions},
  year = 2019,
  eprintclass = {math.NA},
  eprint  =	 {1901.01002}
}

@Article{MezicMauroy,
  author = {Mauroy, I. and Mezi\'{c}},
  title = {Global Stability Analysis Using the Eigenfunctions of the Koopman Operator},
  journal =	{IEEE Transactions on Automatic Control},
  volume  =	61,
  number  =	11,
  year    = 2016,
  pages   =	{3356--3369}
}

@Book{Paulsen,
  author = {Paulsen, V. and Raghupathi, M.},
  title = {An introduction to the theory of reproducing kernel hilbert spaces},
  publisher = {Cambridge studies in advanced mathematics},
  year    = {2016}
}

@Article{Perron-FrobSymmetry,
  author = {Prashant, G. and Hessel-von Molo, M. and M. and Dellnitz, M.},
  title = {Symmetry of attractors and the Perron-Frobenius operator},
  journal =	{Journal of Difference Equations and Applications},
  volume  =	12,
  number  =	11,
  year    = 2006,
  pages   =	{1147--1178}
}

@Article{RosenfeldSystemIdentification,
  author =	 {Rosenfeld, J. A. and Russo, B. and Kamalapurkar, R. and Johnson, T. T.},
  title = {The Occupation Kernel Method for Nonlinear System Identification},
  journal =	{58th Conference on Decision and Control},
  year    = 2019,
  pages   =	 {6455--6460}
 }

@Misc{Rosenfeld,
  author = {Rosenfeld, J. and Kamalapurkar, R. and Forest Gruss, L. and Johnson, T.T.},
  title = {Dynamic Mode Decomposition for Continuous Time Systems with the Liouville Operator},
  year = 2020,
  eprintclass = {math.NA},
  eprint  =	 {1910.03977}
}

@Book{Rudin,
  author = {Rudin, W.},
  title = {Functional analysis},
  publisher = {McGraw-Hill Book Co},
  year    = 1991
}

@Book{SS16,
  author = {Saitoh, S. and Sawano, Y.},
  title = {Theory of reproducing kernel Hilbert spaces},
  publisher = {Development of Mathematics, Springer},
  year    = 2016
}

@Article{Scheffold,
  author = {Scheffold, E.},
  title = {Das Spektrum von Verbandsoperatoren in Banachverbänden},
  journal =	{Mathematische Zeitschrift},
  volume  =	123,
  year    = 1971,
  pages   =	{177--190}
}

@Misc{SparseKoopman,
  author = {Schlosser, C. and Korda, M.},
  title = {Sparsity structures for Koopman operators},
  year = 2021,
  eprintclass = {math.NA},
  eprint  =	 {2112.10887}
}

@Book{SVM2008,
  author = {Steinwart, I. and Christmann, A.},
  title = {Support Vector Machines},
  publisher = {Springer-Verlag New York},
  year    = 2008
}

@Article{EDMD,
  author = {Williams, M.O. and Kevrekidis, I.G. and Rowley, C.W.},
  title = {A Data–Driven Approximation of the Koopman Operator: Extending Dynamic Mode Decomposition},
  journal =	{J. Nonlinear Sci.},
  volume  =	25,
  year    = 2015,
  pages   =	{1307-–1346}
}

@Article{AppliedKoopmanism,
  author =	 {Budisic, M. and Mohr, R. and Mezi\'{c}, I.},
  title = {Applied Koopmanism},
  journal =	{Chaos},
  volume  =	22,
  year    = 2012,
  pages   =	 {047510}
}

@Article{Chen,
  author =	 {Chen, M. and Herbert, S. L. and Vashishtha, M. S. and Bansal, S. and Tomlin, C. J.},
  title = {Decomposition of Reachable Sets and Tubes for a Class of Nonlinear Systems},
  journal =	{IEEE Transactions on Automatic Control},
  volume  =	63,
  number  =	11,
  month   =	11,
  year    = 2018,
  pages   =	 {3675--3688}
}

@Book{OperatorTheoreticAspectsOfErgodicTheory,
  author =	 {Eisner, T. and Farkas, B. and Haase, M. and Nagel, R.},
  title = {Operator Theoretic Aspects of Ergodic Theory},
  publisher = {Berlin, Heidelberg (Springer)},
  year    = 2015
}

@Article{MilanDataDrivenKoopman,
  author =	 {Korda, M. and Putinar, M. and Mezi\'{c}, I.},
  title = {Data-driven spectral analysis of the Koopman operator},
  journal =	{Applied and Computational Harmonic Analysis},
  volume  =	48,
  number  =	2,
  year    = 2020,
  pages   =	 {599--629}
}

@Article{MilanDMD,
  author =	 {Korda, M. and Mezi\'{c}, I.},
  title = {On Convergence of Extended Dynamic Mode Decomposition to the Koopman Operator},
  journal =	{Journal of Nonlinear Science},
  volume  =	28,
  year    = 2018,
  pages   =	 {687–-710}
}

@Article{MilanMPC,
  author =	 {Korda, M. and I. Mezi\'{c}, I.},
  title = {Linear predictors for nonlinear dynamical systems: Koopman operator meets model predictive control},
  journal =	{Automatica},
  volume  =	93,
  year    = 2018,
  pages   =	 {149--160}
}

@Article{MilanEigenfunction,
  author =	 {Korda, M. and Mezi{\'c}, I.},
  title = {Optimal Construction of Koopman Eigenfunctions for Prediction and Control},
  journal =	{IEEE Transactions on Automatic Control},
  volume  =	65,
  year    = 2020,
  pages   =	 {5114--5129}
}

@Article{KariKuester,
  author =	 {K\"{u}ster, K.},
  title = {The Koopman Linearization of Dynamical Systems},
  publisher = {Diplomarbeit},
  year    = 2015
}

@Article{Viktoria,
  author =	 {Kühner, V.},
  title = {What can Koopmanism do for attractors in dynamical systems?},
  journal =	{The Journal of Analysis},
  volume  =	29,
  year    = 2021,
  pages   =	 {449–-471}
}

@Misc{MezicKoopmanOperatorSpectrum,
  author =	 {Mezi\'{c}, I.},
  title = {Koopman Operator Spectrum and Data Analysis},
  year    = 2017,
  eprintclass = {math.NA},
  eprint  =	 {1702.07597}
}

@Article{IgorFluid,
  author =	 {Mezi\'{c}, I.},
  title = {Analysis of fluid flows via spectral properties of the Koopman operator},
  journal =	{Annual review of fluid mechanics},
  volume  =	45,
  year    = 2013,
  pages   =	 {357-–378}
 }

@Article{Symmetry,
  author =	 {Salova, A. and Emenheiser, J. and Rupe, A. and Crutchfield, J. P. and D’Souza, R. M.},
  title = {Koopman operator and its approximations for systems with symmetries},
  journal =	{Chaos},
  volume  =	29,
  year    = 2019,
  pages   =	 {093128}
 }

@Article{SparsePaper,
  author =	 {Schlosser, C. and Korda, M.},
  title = {Sparse moment-sum-of-squares relaxations for nonlinear dynamical systems with guaranteed convergence},
  journal =	{Automatica},
  volume  =	134,
  month   =	12,
  year    = 2021,
  pages   =	 {109900},
 }

@Book{DMDSchmid,
  author =	 {Schmid, P. J.},
  title = {Dynamic mode decomposition of numerical and experimental data},
  publisher = {Cambridge University Press},
  year    = 2010
 }

@Article{KernelMethodsDMD,
    author =	 {Williams, M. O. and Rowley, C. W. and Kevrekidis, I. G.},
    title = {A kernel-based method for data-driven koopman spectral analysis},
    journal =	{Journal of Computational Dynamics},
    volume  =	2,
    number  =	2,
    year    = 2015,
    pages   =	 {247--265}
}

@article {Taniguchi19,
    AUTHOR = {Iwabuchi, Tsukasa and Matsuyama, Tokio and Taniguchi, Koichi},
     TITLE = {Besov spaces on open sets},
   JOURNAL = {Bull. Sci. Math.},
  FJOURNAL = {Bulletin des Sciences Math\'{e}matiques},
    VOLUME = {152},
      YEAR = {2019},
     PAGES = {93--149},
      ISSN = {0007-4497},
   MRCLASS = {46F05 (35J10 81Q10)},
  MRNUMBER = {3904287},
       DOI = {10.1016/j.bulsci.2019.01.008},
       URL = {https://doi-org.kras.lib.keio.ac.jp/10.1016/j.bulsci.2019.01.008},
}
	
@book {Triebelbook,
    AUTHOR = {Triebel, Hans},
     TITLE = {Theory of function spaces},
    SERIES = {Monographs in Mathematics},
    VOLUME = {78},
 PUBLISHER = {Birkh\"{a}user Verlag, Basel},
      YEAR = {1983},
     PAGES = {284},
      ISBN = {3-7643-1381-1},
   MRCLASS = {46Exx},
  MRNUMBER = {781540},
       DOI = {10.1007/978-3-0346-0416-1},
       URL = {https://doi-org.kras.lib.keio.ac.jp/10.1007/978-3-0346-0416-1},
}
@article{Xia-2019,   
   author={Xiao, Jie},
   title={The transport equation in the scaling invariant Besov or
   Ess\'{e}n-Janson-Peng-Xiao space},
   journal={J. Differential Equations},
   volume={266},
   date={2019},
   number={11},
   pages={7124--7151},
  issn={0022-0396},
  review={\MR{3926095}},
  doi={10.1016/j.jde.2018.11.027},
}

@article{fixman1959problems,
  title={Problems in spectral operators.},
  author={Fixman, Uri},
  journal={Pacific Journal of Mathematics},
  volume={9},
  number={4},
  pages={1029--1051},
  year={1959},
  publisher={Pacific Journal of Mathematics, A Non-profit Corporation}
}

@article{dogra2020optimizing,
  title={Optimizing neural networks via Koopman operator theory},
  author={Dogra, Akshunna S and Redman, William},
  journal={Advances in Neural Information Processing Systems},
  volume={33},
  pages={2087--2097},
  year={2020}
}

@article{russo2022liouville,
  title={Liouville operators over the Hardy space},
  author={Russo, Benjamin P and Rosenfeld, Joel A},
  journal={Journal of Mathematical Analysis and Applications},
  volume={508},
  number={2},
  pages={125854},
  year={2022},
  publisher={Elsevier}
}

@article{rosenfeld2022dynamic,
  title={Dynamic mode decomposition for continuous time systems with the Liouville operator},
  author={Rosenfeld, Joel A and Kamalapurkar, Rushikesh and Gruss, L and Johnson, Taylor T},
  journal={Journal of Nonlinear Science},
  volume={32},
  number={1},
  pages={1--30},
  year={2022},
  publisher={Springer}
}

@article{menovschikov2021composition,
  title={Composition operators on Sobolev spaces, $ Q $-mappings and weighted Sobolev inequalities},
  author={Menovschikov, Alexander and Ukhlov, Alexander},
  journal={arXiv preprint arXiv:2110.09261},
  year={2021}
}

@article{dette2021reproducing,
  title={Reproducing kernel Hilbert spaces, polynomials, and the classical moment problem},
  author={Dette, Holger and Zhigljavsky, Anatoly A},
  journal={SIAM/ASA Journal on Uncertainty Quantification},
  volume={9},
  number={4},
  pages={1589--1614},
  year={2021},
  publisher={SIAM}
}

@inproceedings{mukherjee2011range,
  title={On the range of composition operators on spaces of entire functions},
  author={Mukherjee, S and Jafari, F and McInroy, JE},
  booktitle={Function Spaces in Modern Analysis: Sixth Conference on Function Spaces, May 18-22, 2010, Southern Illinois University, Edwardsville},
  volume={547},
  pages={185},
  year={2011},
  organization={American Mathematical Soc.}
}

@article{bergner2006spectral,
  title={A spectral analysis of function composition and its implications for sampling in direct volume visualization},
  author={Bergner, Steven and Moller, Torsten and Weiskopf, Daniel and Muraki, David J},
  journal={IEEE transactions on visualization and computer graphics},
  volume={12},
  number={5},
  pages={1353--1360},
  year={2006},
  publisher={IEEE}
}

@article{lebedev2012functions,
  title={On-functions with bounded spectrum},
  author={Lebedev, Vladimir V},
  journal={Sbornik: Mathematics},
  volume={203},
  number={11},
  pages={1647},
  year={2012},
  publisher={IOP Publishing}
}

@inproceedings{azizi1999preservation,
  title={On the preservation of bandlimitedness under non-affine time warping},
  author={Azizi, Shahrnaz and Cochran, Douglas and McDonald, John N},
  booktitle={Proc. Int. Workshop on Sampling Theory and Applications},
  pages={37--40},
  year={1999}
}

@article{sriperumbudur2011universality,
  title={Universality, Characteristic Kernels and RKHS Embedding of Measures.},
  author={Sriperumbudur, Bharath K and Fukumizu, Kenji and Lanckriet, Gert RG},
  journal={Journal of Machine Learning Research},
  volume={12},
  number={7},
  year={2011}
}

@article{alexander2020operator,
  title={Operator-theoretic framework for forecasting nonlinear time series with kernel analog techniques},
  author={Alexander, Romeo and Giannakis, Dimitrios},
  journal={Physica D: Nonlinear Phenomena},
  volume={409},
  pages={132520},
  year={2020},
  publisher={Elsevier}
}
@article{das2021reproducing,
  title={Reproducing kernel Hilbert space compactification of unitary evolution groups},
  author={Das, Suddhasattwa and Giannakis, Dimitrios and Slawinska, Joanna},
  journal={Applied and Computational Harmonic Analysis},
  volume={54},
  pages={75--136},
  year={2021},
  publisher={Elsevier}
}

@article{lian2021koopman,
  title={Koopman based data-driven predictive control},
  author={Lian, Yingzhao and Wang, Renzi and Jones, Colin N},
  journal={arXiv preprint arXiv:2102.05122},
  year={2021}
}
